A Sequential Homotopy Method for Mathematical Programming Problems

We propose a sequential homotopy method for the solution of mathematical programming problems formulated in abstract Hilbert spaces under the Guignard constraint qualification. The method is equivalent to performing projected backward Euler timestepping on a projected gradient/antigradient flow of the augmented Lagrangian. The projected backward Euler equations can be interpreted as the necessary optimality conditions of a primal-dual proximal regularization of the original problem. The regularized problems are always feasible, satisfy a strong constraint qualification guaranteeing uniqueness of Lagrange multipliers, yield unique primal solutions provided that the stepsize is sufficiently small, and can be solved by a continuation in the stepsize. We show that equilibria of the projected gradient/antigradient flow and critical points of the optimization problem are identical, provide sufficient conditions for the existence of global flow solutions, and show that critical points with emanating descent curves cannot be asymptotically stable equilibria of the projected gradient/antigradient flow, practically eradicating convergence to saddle points and maxima. The sequential homotopy method can be used to globalize any locally convergent optimization method that can be used in a homotopy framework. We demonstrate its efficiency for a class of highly nonlinear and badly conditioned control constrained elliptic optimal control problems with a semismooth Newton approach for the regularized subproblems. In contrast to the published article, this version contains a correction that the associate editor considers as too insignificant to justify publication in the journal.

==> pendulum.tex <==
% Contents of supplementary material.

\begin{figure}[p]
  \centering
  \input{pendulum_x}
  \hfill
  \input{pendulum_y}
  \caption{Primal (left) and dual (right) trajectories of the
    gradient/antigradient flow of the augmented Lagrangian for the pendulum
    of Example~\ref{ex:pendulum}. The initial value is $x_1 = 0.01$,
    $x_2 = 1$, $y=-\smash[b]{\frac{1}{2}}$, which is close to the inverted
    pendulum position. For larger values of the penalty parameter $\rho$, the
    primal trajectories are driven closer to the feasible set ($\norm{x}{2} =
    1$), but the dual trajectories converge more slowly to the minimum.}
    %$x_1 = 0$, $x_2 = -1$, $y = \smash[b]{\frac{1}{2}}$.}
  \label{fig:pendulum}
\end{figure}

\begin{figure}[p]
  \centering
  \input{pendulum_streamlines_max}
  \hfill
  \input{pendulum_streamlines_min}
  \hfill
  \input{pendulum_streamlines_newton}
  \caption{Primal streamlines of the gradient/antigradient and the Newton flow
    for the pendulum of Example~\ref{ex:pendulum} for $\rho = 1$. The
    maximum is marked by $\times$ and the minimum by $+$. The primal streamlines
    are given for the Lagrange multipliers corresponding to the maximum
    ($y=\smash[b]{-\frac{1}{2}}$) and the minimum ($y=\smash[b]{\frac{1}{2}}$).
    The maximum is not stable for the gradient/antigradient flow (left), the
    minimum is stable for the gradient/antigradient flow (middle), and the
    maximum is stable for the Newton flow (right). Moreover, the Newton flow is
    not defined on the circle with radius $\sqrt{1.5}$, where the Hessian of the
    augmented Lagrangian is singular.}
  \label{fig:pendulum_streamlines}
\end{figure}

\begin{figure}[p]
  \centering
  \input{pendulum_backward_euler}
  \caption{Relative errors of backward Euler timestepping with timestep $\Delta
    t = 10^{0}, 10^{1}, \dotsc, 10^{8}$ for the gradient/antigradient flow of
    the augmented Lagrangian with $\rho = 1$ for the pendulum of
    Example~\ref{ex:pendulum}. The initial value $x_1 = 0.01$, $x_2 = 1$, $y =
    -\smash[b]{\frac{1}{2}}$ is close to the maximum. The errors converge
    linearly to zero with a rate very close to the timestep $\Delta t$. We
    solved each time step by a numerical homotopy method in $\Delta t$.}
  \label{fig:pendulum_backward_euler}
\end{figure}

%\afterpage{\clearpage}

\begin{example}[Kinematic pendulum model]
  \label{ex:pendulum}
  Let a point mass be fixed at the end of a massless rod rotating about its
  other fixed end. We would like to determine the position of minimal potential
  energy. Disregarding physical quantities and units, this leads to an
  optimization problem of the form
  \begin{equation}
    \label{eqn:pendulum_mp}
    \min \phi(x) = x_2 \quad \text{over } x \in \mathbb{R}^2 
    \quad \text{subject to } c(x) = x_1^2 + x_2^2 - 1 = 0,
  \end{equation}
  with corresponding Lagrangian $L^{0}(x, y) = \phi(x) + y c(x)$.
  By standard NLP theory, the necessary optimality conditions imply that
  $x_1 = 0$, $x_2 = \pm 1$, $y = \mp \smash[b]{\frac{1}{2}}$ must hold at a
  solution, where the upper critical point ($x_2 = 1$,
  $y=-\smash[b]{\frac{1}{2}}$) is a maximum and the lower critical point ($x_2 =
  -1$, $y=\smash[b]{\frac{1}{2}}$) is the only minimum,
  which corresponds to the rod being balanced upwards or hanging down. We
  construct a gradient/antigradient flow for this problem, for which all
  critical points are equilibria, but the maximum is unstable and the minimum is
  stable: Adding an augmented Lagrangian term to the objective $\phi^{\rho}(x) =
  x_2 + \frac{\rho}{2} c^2(x)$, $\rho \ge 0$, we can consider moving along the
  negative gradient with respect to the primal variables and the positive
  gradient with respect to the dual variables of the augmented
  Lagrangian function $L^{\rho}(x, y) = \phi^{\rho}(x) + y c(x)$ with the
  differential equation
  \begin{align*}
    \dot{x}_1(t) &= -\nabla_{x_1} L^{\rho}(x(t), y(t))
    = -2[y(t) + \rho c(x(t))] x_1(t), \\
    \dot{x}_2(t) &= -\nabla_{x_2} L^{\rho}(x(t), y(t))
    = -2[y(t) + \rho c(x(t))] x_2(t) - 1, \\
    \dot{y}(t) &= +\nabla_{y} L^{\rho}(x(t), y(t)) = c(x(t))
    = x_1(t)^2 + x_2(t)^2 - 1.
  \end{align*}
  We depict solutions of these flow equations for the initial values $x_1 =
  0.01$, $x_2 = 1$, $y = -\frac{1}{2}$ and varying values of $\rho$ in
  Figure~\ref{fig:pendulum}. We see that the flow is in general infeasible for
  the equality constraints, but we can drive the flow closer to the feasible set
  by increasing $\rho$. The streamline plots in
  Figure~\ref{fig:pendulum_streamlines} show that the upper critical point is
  not a stable equilibrium, while the lower one is stable for the
  gradient/antigradient flow. Thus, small perturbations will let us escape the
  maximum (i.e., the position of the inverted pendulum) and eventually lead us
  to the minimum. This is in stark contrast to the Newton flow of the necessary
  optimality conditions $\nabla L^{\rho}(x, y) = 0$, which can formally be
  derived by performing a Newton method on these equations with infinitesimal
  step sizes: The Newton flow, while having nice affine invariance properties,
  is attracted to the maximum, a clearly unwanted critical point
  of~\eqref{eqn:pendulum_mp}.

  For the gradient/antigradient flow, we can perform backward Euler timestepping
  with stepsize $\Delta t > 0$ from a current point $(\hat{x}, \hat{y})$ to
  $(x, y)$ by solving
  \begin{align*}
    x - \hat{x} + \Delta t \nabla_{x} L^{\rho}(x, y) &= 0, &
    y - \hat{y} - \Delta t \nabla_{y} L^{\rho}(x, y) &= 0,
  \end{align*}
  which, with $w = -\Delta t c(x)$, happen to be the necessary
  optimality conditions of
  \[
    \min \phi^{\rho}(x) + \lambda \left[ \tfrac{1}{2} \norm{x - \hat{x}}{2}^2 +
    \norm{w - \hat{y}}{2}^2 \right] \quad \text{over } (x, w) \in
    \mathbb{R}^{2+1} 
    \quad \text{s.t.~} c(x) + \lambda w = 0,
  \]
  where $\lambda = \frac{1}{\Delta t}$. This proximally regularized problem is
  always feasible, satisfies the linear independence constraint qualification in
  all its feasible points, and its solution can be traced numerically by a
  homotopy method for decreasing $\lambda$. This is the basic idea of the
  sequential homotopy method proposed here. 
  While it cannot be guaranteed that we can drive $\lambda$ arbitrarily close to
  zero, i.e., $\Delta t \to \infty$, we can stop at some $\lambda > 0$ and
  accept the solution as a backward Euler step of the gradient/antigradient
  flow.  For small values of $\Delta t$ (large $\lambda$), the Lagrangian
  Hessian of the proximally regularized problem is guaranteed to be positive
  definite. For large values of $\Delta t$ (small $\lambda$), fast convergence
  of the method can be recovered locally (compare
  Figure~\ref{fig:pendulum_backward_euler}).
\end{example}

The up to here admittedly unmotivated use of the augmentation term is important
to guarantee convergence of the flow, but larger penalization coefficients will
generate fast transients towards the feasible set and thus cause increased
stiffness of the flow equations, which the following small example demonstrates:

\begin{example}
  Consider the nonconvex constrained scalar problem
  \[
    \min \phi(x) = -\tfrac{1}{2} x^2 \quad \text{over } x \in \mathbb{R}
    \quad \text{subject to } x = 0.
  \]
  Its solution is its only feasible point $x=0$ with Lagrange multiplier $y=0$.
  The gradient/antigradient flow for the augmented Lagrangian reduces to the
  homogeneous linear ordinary differential equation
  \[
    \begin{pmatrix}
      \dot{x}(t)\\
      \dot{y}(t)
    \end{pmatrix}
    =
    \begin{pmatrix}
      1 - \rho & ~ & -1\\
      1 & &  0
    \end{pmatrix}
    \begin{pmatrix}
      x(t)\\
      y(t)
    \end{pmatrix},
  \]
  whose system matrix has the eigenvalues $\mu_{1,2} = \frac{1}{2} \left(
  \pm \sqrt{(\rho+1)(\rho-3)} + 1 - \rho \right)$. We immediately see that for
  $\rho \le 3$, the real parts are $1 - \rho$, so we need $\rho > 1$ to
  guarantee stability. For $\rho \ge 3$, both eigenvalues are negative reals and
  their asymptotics are $\mu_1 \to 0$ and $\mu_2 \to -\infty$,
  so that the gradient/antigradient flow is stable but the equations become
  increasingly stiff for $\rho \to \infty$.
\end{example}

% vim: ts=8 sw=2

